Error Correction for Reliable Quantum Computing

Quantum computers herald the arrival of a new era in which previously intractable computational problems will be solved efficiently. However, quantum technology is held down by decoherence, a phenomenon that is omnipresent in the quantum paradigm and that renders quantum information useless when left unchecked. The science of quantum error correction, a discipline that seeks to combine and protect quantum information from the effects of decoherence using structures known as codes, has arisen to meet this challenge. Stabilizer codes, a particular subclass of quantum codes, have enabled fast progress in the field of quantum error correction by allowing parallels to be drawn with the widely studied field of classical error correction. This has resulted in the construction of the quantum counterparts of well-known capacity-approaching classical codes like sparse codes and quantum turbo codes. However, quantum codes obtained in this manner do not entirely evoke the stupendous error correcting abilities of their classical counterparts. This occurs because classical strategies ignore important differences between the quantum and classical paradigms, an issue that needs to be addressed if quantum error correction is to succeed in its battle with decoherence. In this dissertation we study a phenomenon exclusive to the quantum paradigm, known as degeneracy, and its effects on the performance of sparse quantum codes. Furthermore, we also analyze and present methods to improve the performance of a specific family of sparse quantum codes in various different scenarios.

==> Texs/BIB/biblio3.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\begin{thebibliography}{9}	

\bibitem{feynman} R. P. Feynman, ``Simulating physics with computers,'' \textit{Int. J. Theor. Phys.}, vol. 21, pp. 467-488, 1982. doi: 10.1007/BF02650179.


\bibitem{bab1}  S. Imre and F. Balazs, ``Quantum Computing and Communications: An Engineering Approach,'' \textit{John Wiley \& Sons}, 2005. ISBN:978-0-470-86902-4.


\bibitem{bab2} D. Deutsch and R. Jozsa, ``Rapid solution of problems by quantum computation,'' \textit{Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}, vol. 439, no. 1907, pp. 553-558, 1992. doi: https://doi.org/10.1098/rspa.1992.0167.

\bibitem{shor} P. W. Shor, ``Polynomial-Time Algorithms for Prime Factorization and Discrete Logarithms on a Quantum Computer,'' \textit{SIAM Journal on Computing}, vol. 26, no. 5, pp. 1484-1509, 1997. doi: 	10.1137/S0097539795293172.

\bibitem{grover1} L. K. Grover, ``A Fast Quantum Mechanical Algorithm for Database Search,'' \textit{Annual ACM Symp. on Theory of Comp.}, pp. 212-219, 1996. arXiv:quant-ph/9605043.

\bibitem{grover2} L. K. Grover, ``From Schrodingers equation to the quantum search algorithm,'' \textit{Pramana - J. Phys.}, vol. 56, pp. 333-348, 2001. doi: 10.1007/s12043-001-0128-3.

\bibitem{byzantine} M. Fitzi, N. Gisin, and U. Maurer, ``Quantum Solution to the Byzantine Agreement Problem,'' \textit{Phys. Rev. Lett.}, vol. 87, no. 21, pp. 217901, 2001. doi: 10.1103/PhysRevLett.87.217901.

\bibitem{parallel1} D. Alanis, P. Botsinis, S. X. Ng, and L. Hanzo, ``Quantum-assisted
routing optimization for self-organizing networks,'' \textit{IEEE Access }, vol. 2, pp. 614-632, 2014. doi: 10.1109/ACCESS.2014.2327596.

\bibitem{parallel2} D. Alanis, P. Botsinis, Z. Babar, S. X. Ng, and L. Hanzo, ``Non-dominated
quantum iterative routing optimization for wireless multihop networks,'' \textit{IEEE Access}, vol. 3, pp. 1704-1728, 2015. doi: 10.1109/ACCESS.2015.2478793.

\bibitem{parallel3} P. Botsinis, D. Alanis, Z. Babar, S. X. Ng, and L. Hanzo, ``Noncoherent
quantum multiple symbol differential detection for wireless systems,'' \textit{IEEE Access}, vol. 3, pp. 569-598, 2015. doi: 10.1109/ACCESS.2015.2432015.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 11 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{BB84} C. H. Bennett, and G. Brassard, ``Quantum cryptography: Public key distribution and coin tossing
,'' \textit{Theoretical Computer Science}, vol. 560, pp. 7-11, 2014. doi: 10.1016/j.tcs.2014.05.025.

\bibitem{E91} A. Ekert, ``Quantum cryptography based on Bells theorem,'' \textit{Phys. Rev. Lett.}, vol. 67, no. 6, pp. 661-663, 1991. doi: 10.1103/PhysRevLett.67.661.

\bibitem{decoherence1} P. W. Shor, ``Scheme for reducing decoherence in quantum computer memory,'' \textit{Phys. Rev. A}, vol. 52, no. 4, pp. R2493-R2496, 1995. doi: 10.1103/PhysRevA.52.R2493.

\bibitem{decoherence2} M. Schlosshauer, ``Decoherence, the measurement problem, and interpretations of quantum mechanics,'' \textit{Rev. Mod. Phys.}, vol. 76, pp. 1267, 2005. doi: 10.1103/RevModPhys.76.1267.

\bibitem{decoherence3} M. Schlosshauer, ``Quantum decoherence,'' \textit{Physics Reports}, vol. 831, pp. 1-57, 2019. doi: 10.1016/j.physrep.2019.10.001.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 16 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{QSC} D. Gottesman, ``Stabilizer codes and quantum error correction,'' \textit{PhD dissertation}, California Inst. Tech., Pasadena, CA, USA, 1997. arXiv:quant-ph/9705052.


\bibitem{QRM} A. M. Steane, ``Quantum Reed Muller codes,'' \textit{IEEE Trans. Inf. Theory}, vol. 45, no. 4, pp. 1701-1703, 1999. doi: 10.1109/18.771249.


\bibitem{bicycle} D. J. C. MacKay, G. Mitchinson, and P. L. McFadden, ``Sparse-graph
codes for quantum error correction,'' \textit{IEEE Trans. Inf. Theory}, vol. 50, no. 10, pp.  2315-2330, 2004. doi: 10.1109/TIT.2004.834737.

\bibitem{qldpc1} T. Camara, H. Ollivier, and J.-P. Tillich, ``Constructions and performance of classes of quantum LDPC codes,'' 2005. arXiv:quant-ph/0502086.

\bibitem{qldpc15} Z. Babar, P. Botsinis, D. Alanis, S. X. Ng, and L. Hanzo, ``Fifteen Years of Quantum LDPC Coding and Improved Decoding Strategies,'' \textit{IEEE Access}, vol. 3, pp. 2492-2519, 2015. doi. 10.1109/ACCESS.2015.2503267.

\bibitem{jgf1} H. Lou, and J. Garcia-Frias ``Quantum error-correction using codes with low-density generator matrix,'' \textit{IEEE 6th Workshop on Signal Processing Advances in Wireless Communications}, 2005. doi: 10.1109/SPAWC.2005.1506298. 

\bibitem{jgf2} 
H. Lou and J. Garcia-Frias, ``On the Application of Error-Correcting Codes with Low Density Generator Matrix over Different Quantum Channels,'' \textit{4th International Symposium on Turbo Codes \& Related Topics}, 2006. online: https://ieeexplore.ieee.org/document/5755950.

\bibitem{patrick} P. Fuentes, J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Frias, ``Approach for the construction of non-Calderbank-Steane-Shor low-density-generator-matrix based quantum codes,'' \textit{Phys. Rev. A}, vol. 102, pp. 012423, 2020. doi: 10.1103/PhysRevA.102.012423.

\bibitem{patrick-asym} P. Fuentes, J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Frias, ``Design of low-density-generator-matrix--based quantum codes for asymmetric quantum channels,'' \textit{Phys. Rev. A}, vol. 103, pp. 022617, 2021. doi: 10.1103/PhysRevA.103.022617.

\bibitem{QCC1} H. Ollivier, and J. P. Tillich, ``Description of a quantum convolutional code,'' \textit{Phys. Rev. Lett.}, vol. 91, 2003. doi: 	10.1103/PhysRevLett.91.177902.

\bibitem{QCC2} M. Grassl and M. Rotteler, ``Non-catastrophic en-
coders and encoder inverses for quantum convolutional
codes,'' \textit{Proc. ISIT IEEE}, pp. 1019, 2006. doi: 10.1109/ISIT.2006.261956.

\bibitem{QCC3} J. G. D. Forney, M. Grassl, and S. Guha, ``Con-
volutional and tail-biting quantum error-correcting codes,'' \textit{IEEE Trans. on Inf. Theory}, vol. 53, no. 3, pp. 865-880, 2007. doi: 10.1109/TIT.2006.890698.

\bibitem{QTC} D. Poulin, J. P. Tillich, and  H. Ollivier, ``Quantum Serial Turbo Codes,'' \textit{IEEE Trans. Inf. Theory}, vol. 55, no. 6, pp.  2776-2798, 2009. doi: 10.1109/TIT.2009.2018339.

\bibitem{EAQTC} M. M. Wilde, M. Hsieh, and  Z. Babar, ``Entanglement-Assisted Quantum Turbo Codes,'' \textit{IEEE Trans. Inf. Theory}, vol. 60, no. 2, pp.  1203-1222, 2014. doi: 10.1109/TIT.2013.2292052.

\bibitem{josu1} J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Fr\'ias, ``On the Performance of Interleavers for Quantum Turbo Codes,'' \textit{Entropy}, vol. 21, no. 7, pp. 633, 2019. doi: 10.3390/e21070633.

\bibitem{josu2} J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Fr\'ias, ``Depolarizing Channel Mismatch and Estimation Protocols for Quantum Turbo Codes,'' \textit{Entropy}, vol. 21, no. 12, pp. 1133, 2019. doi: 10.3390/e21121133.

\bibitem{toric} A. Y. Kitaev, ``Quantum computations: Algorithms and error correction,'' \textit{Russ. Math. Surveys}, vol. 52, no. 6, pp. 1191-1249, 1997. doi: 10.1070/rm1997v052n06abeh002155.

\bibitem{top1} E. Dennis, A. Kitaev, A. Landahl, and J. Preskill,
``Topological quantum memory,'' \textit{J. Math. Phys.}, vol. 43, pp. 4452-4505, 2002. doi: 10.1063/1.1499754.

\bibitem{top2} A. Y. Kitaev, ``Fault-tolerant quantum computation by anyons,'' \textit{Ann. Phys.}, vol. 303, pp. 2, 2003. doi: 10.1016/S0003-4916(02)00018-0.

\bibitem{surface} A. G. Fowler, M. Mariantoni, J. M. Martinis, A. N. Cleland, ``Surface codes: Towards practical large-scale quantum computation,'' \textit{Phys. Rev. A}, vol. 86, pp. 032324, 2012. doi: 10.1103/PhysRevA.86.032324.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 36 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{threshold} D. Aharonov, and M. Ben-Or, ``Fault-tolerant quantum computation with constant error,'' \textit{Proceedings of the twenty-ninth annual ACM symposium on Theory of computing}, pp. 176--188, 1997. online: 	arXiv:quant-ph/9611025. 

\bibitem{fault1} E. Knill, R. Laflamme, and W. H. Zurek, ``Resilient quantum computation: Error Models and Thresholds,'' \textit{Proc. Roy. Soc. A}, vol. 454, pp. 342, 1998. doi: 10.1098/rspa.1998.0166.

\bibitem{fault2} R. Laflamme, C. Miquel, J. P. Paz, and W. H.
Zurek, ``Perfect quantum error correction code,'' \textit{Phys. Rev. Lett.}, vol. 77, pp. 198, 1996. doi: 10.1103/PhysRevLett.77.198.

\bibitem{fault3} J. Preskill, ``Fault-tolerant quantum computation,'' \textit{Introduction to quantum computation}, 1999. arXiv:quant-ph/9712048.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 40 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{ref1} J. Tillich and G. Zémor, ``Quantum LDPC Codes With Positive Rate and Minimum Distance Proportional to the Square Root of the Blocklength,'' \textit{IEEE Transactions on Information Theory}, vol. 60, no. 2, pp. 1193-1202, 2014. doi: 10.1109/TIT.2013.2292061.

\bibitem{ref2} A. Leverrier, J. Tillich and G. Zémor, ``Quantum Expander Codes,'' \textit{2015 IEEE 56th Annual Symposium on Foundations of Computer Science}, pp. 810-824, 2015. doi: 10.1109/FOCS.2015.55.

\bibitem{ref3} M. B. Hastings, J. Haah, and R. O'Donnell, ``Fiber Bundle Codes: Breaking the $N^{\frac{1}{2}}$ polylog($N$) Barrier for Quantum LDPC Codes,'' 2020. arXiv:2009.03921.

\bibitem{ref4} P. Panteleev and G. Kalachev, ``Quantum LDPC Codes with Almost Linear Minimum Distance,'' 2020. arXiv:2012.04068.

\bibitem{ref5} N. P. Breuckmann, J. N. Eberhardt, ``Balanced Product Quantum Codes,'' 2020. arXiv:2012.09271.

\bibitem{ref6} N. P. Breuckmann, J. N. Eberhardt, ``Homological product codes,'' \textit{Proceedings of the forty-sixth annual ACM symposium on Theory of computing (STOC '14)}, pp. 273–282., 2014. doi: 10.1145/2591796.2591870.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 46 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{turbo} 
C. Berrou, A. Glavieux, and P. Thitimajshima, ``Near Shannon limit error-correcting coding and decoding: Turbo-codes,'' \textit{Proceedings of ICC '93 - IEEE International Conference on Communications}, vol. 2, pp. 1064-1070, 1993. doi: 10.1109/ICC.1993.397441.

\bibitem{spa} 
F.R. Kschischang, B.J. Frey, and H.A. Loeliger, ``Factor graphs and the sum-product algorithm,'' \textit{IEEE Transactions on Information Theory},  vol.47, no. 2, pp. 498--519, 2001. doi: 10.1109/18.910572.

\bibitem{BP} 
J. Pearl, ``Probabilistic Reasoning in Intelligent Systems: Networks of Plausible Inference,'' \textit{Morgan Kauffman}, 1988. online: https://www.sciencedirect.com/book/9780080514895/probabilistic-reasoning-in-intelligent-systems.

\bibitem{Viterbi} 
G. D. Forney, ``The Viterbi Algorithm,'' \textit{Proceedings of the IEEE},  vol.61, no. 3, pp. 268-278 1973. doi: 10.1109/PROC.1973.9030

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 50 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Wiberg}
N.Wiberg, ``Codes and decoding on general graphs,'' \textit{PhD dissertation}, 1996. online: https://www.semanticscholar.org/paper/Codes-and-Decoding-on-General-Graphs-Wiberg/eb44d50bce92b4ce2c0ea53bd8ede95f628ee3cb.

\bibitem{qBP1} 
M. B. Hastings, ``Quantum belief propagation,'' \textit{Phys. Rev. B}, vol.76, pp. 201102, 2007. doi: 10.1103/PhysRevB.76.201102.

\bibitem{qBP2} 
M. Leifer and D. Poulin, ``Quantum graphical models
and belief propagation,'' \textit{Annals of Physics},  vol.323, no. 8, pp. 1899-1946, 2007. doi: 10.1016/j.aop.2007.10.001

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 53 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{degen1} 
D. P. DiVincenzo, P. W. Shor, and J. A. Smolin, ``Quantum-channel capacity of very noisy channels,'' \textit{Phys.
Rev. A}, vol.57, pp. 830-839, 1998. doi: 10.1103/PhysRevA.57.830.

\bibitem{degen2} 
G. Smith and J. A. Smolin, ``Degenerate Quantum Codes for Pauli Channels,'' \textit{Phys. Rev. Lett.},  vol.98, pp. 030501, 2007. doi: 10.1103/PhysRevLett.98.030501.

\bibitem{degen3} 
D. Poulin and Y. Chung, ``On the iterative decoding of sparse quantum codes,'' \textit{QIC}, vol.8, no.10 pp. 987, 2008. doi: 10.5555/2016985.2016993.

\bibitem{degen4} 
M. H. Hsieh and F. Le Gall, ``NP-hardness of decoding quantum error-correction codes,'' \textit{Phys. Rev. A}, vol. 83, pp. 052331, 2010. doi: 10.1103/PhysRevA.83.052331.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 57 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{CSS1} 
A. R. Calderbank and P. W. Shor, ``Good quantum error correcting codes exist,'' \textit{Physical Review A}, vol. 54, pp. 1098-1105, 1996. doi: 10.1103/PhysRevA.54.1098.

\bibitem{CSS2} 
A. Steane, Proceedings of The Royal Society A Mathematical, ``Multiple-particle interference and quantum error correction,'' \textit{Physical and Engineering Sciences}, vol. 452, no. 1954, 1996. doi: 10.1098/rspa.1996.0136.

\bibitem{EA1} 
M-H. Hsieh, I. Devetak, and T. Brun, ``General entanglement-assisted quantum error-correcting codes,'' \textit{Physical Review A}, vol. 76, pp. 062313, 2007. doi: 10.1103/PhysRevA.76.062313.

\bibitem{EA2} 
M-H. Hsieh, T. Brun, and I. Devetak, ``Entanglement-assisted quantum quasicyclic low-density parity-check codes,'' \textit{Physical Review A}, vol. 79, pp. 032340, 2009. doi: DOI:10.1103/PhysRevA.79.032340.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 61 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{EA3} 
Y. Fujiwara and V. D. Tonchev, ``A Characterization of Entanglement-Assisted Quantum Low-Density Parity-Check Codes,'' \textit{IEEE Transactions on Information Theory}, vol. 59, no. 6, pp. 3347-3353. doi: 10.1109/TIT.2013.2247461.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 62 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{CSSbound} 
D. Maurice, J.-P. Tillich, and I. Andriyanova, ``A family of quantum codes with performances close to the hashing bound under iterative decoding,'' \textit{IEEE International Symposium on Information Theory}, pp. 907-911, 2013. doi: 10.1109/ISIT.2013.6620358.2013.

\bibitem{nonCSS1} 
T. Camara, H. Ollivier, and J.-P. Tillich, ``A class of quantum LDPC codes: construction and performances under iterative decoding,'' \textit{IEEE International Symposium on Information Theory}, pp. 811-815, 2007. doi: 10.1109/ISIT.2007.4557324.

\bibitem{nonCSS2} 
D. Maurice, J.-P. Tillich, and I. Andriyanova, ``Spatially coupled quantum LDPC codes,'' \textit{IEEE Information Theory Workshop}, 2012. doi: 10.1109/ITW.2012.6404686.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 65 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{symplec1} A. R. Calderbank and P. W. Shor, ``Good quantum error correcting codes exist,'' \emph{Phys. Rev. A}, vol. 54, pp. 1098-1105, 1996. doi: 10.1103/PhysRevA.54.1098.

\bibitem{symplec2} A. R. Calderbank, E. M. Rains, P. W. Shor, and N. J. A. Sloane, ``Quantum error correction via codes over GF(4),'' \emph{IEEE Trans. Inf. Theory}, vol. 44, pp.1369–1387, 1998. doi: 10.1109/18.681315.

\bibitem{logical}
B. Yoshida and I. L. Chuang, ``Framework for classifying logical operators in stabilizer codes,'' \textit{Phys. Rev. A}, vol. 81, pp. 052302, 2010. doi: 10.1103/PhysRevA.81.052302.

\bibitem{softVit}
E. Pelchat and D. Poulin, ``Degenerate Viterbi Decoding,'' \textit{IEEE Trans. on Information Theory}, vol. 59, no. 6, pp. 3915 - 3921, 2013. doi: 10.1109/TIT.2013.2246815.

\bibitem{neural}
S. Varsamopoulos, B. Criger, and K. Bertels, ``Decoding small surface codes with feedforward neural networks,'' \textit{Quantum Science and Technology}, vol. 3, no. 1, pp. 015004, 2017. doi: 10.1088/2058-9565/aa955a. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 70 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Hard} 
P. Iyer and D. Poulin, ``Hardness of decoding quantum stabilizer codes,'' \textit{IEEE Trans. on Information Theory}, vol. 61, no. 9, pp. 5209-5223, 2015. doi: 10.1109/TIT.2015.2422294.

\bibitem{softPoul}
D. Poulin, ``Optimal and Efficient Decoding of Concatenated Quantum Block Codes,'' \textit{Phys. Rev. A}, vol. 74, pp. 052333, 2006. doi: 10.1103/PhysRevA.74.052333.

\bibitem{toricphd1} D. K. Tuckett, A. S. Darmawan, T. C. Chubb, S. Bravyi, S. D. Bartlett, and S. T. Flammia, ``Tailoring Surface Codes for Highly Biased Noise,'' \textit{Phys. Rev. X}, vol. 9, no. 4, pp. 041031, 2019. doi: 10.1103/PhysRevX.9.041031.

\bibitem{toricphd2} D. K. Tuckett, ``Tailoring surface codes: Improvements in quantum error correction with biased noise,'' \textit{PhD Dissertation}, University of Sydney, 2020.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 74 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{sabo} E. Sabo, A. B. Aloshious, and K. R. Brown, ``Trellis Decoding For Qudit Stabilizer Codes And Its Application To Qubit Topological Codes,'' arXiv:2106.08251, 2021.

\bibitem{NielsenChuang} M. A. Nielsen, and I. Chuang, ``Quantum Computation and Quantum Information: 10th Anniversary Edition,'' \textit{Cambridge: Cambridge University Press}, 2011. doi: 10.1017/CBO9780511976667.

\bibitem{cp1_Gamal} A. E. Gamal and Y-H. Kim. ``Network Information Theory,'' Cambridge University Press, 2012. USA. arXiv: 1001.3404.

\bibitem{Turing}
A. M. Turing, ``On Computable Numbers, with an Application to the Entscheidungsproblem,'' \textit{Proc. Lond. Math. Soc.}, vol. 2, no. 42, pp. 230, 1937. doi: 10.1112/plms/s2-42.1.230.

\bibitem{RSA}
R. L. Rivest, A. Shamir, and L. Adleman, ``A method for obtaining digital signatures and public-key cryptosystems,'' \textit{Communications of the ACM}, vol. 21, no. 2, pp. 120–126, 1978. doi: 10.1145/359340.359342.

\bibitem{ecc}
J. W. Bos, J. A. Halderman, N. Heninger, J. Moore, M. Naehrig, and E. Wustrow E, ``Elliptic Curve Cryptography in Practice,'' \textit{International Conference on Financial Cryptography and Data Security}, pp. 157-175, Springer, Berlin, 2014. doi: 10.1007/978-3-662-45472-5\_11.

\bibitem{bitcoin}
Satoshi Nakamoto, ``Bitcoin : A Peer-to-Peer Electronic Cash System,'' 2009. online: https://bitcoin.org/bitcoin.pdf.

\bibitem{supremacy}
Google Quantum AI, ``Exponential suppression of bit or phase errors with cyclic error correction,'' \textit{Nature}, vol. 595, pp. 383–387, 2021. doi: 10.1038/s41586-021-03588-y.

\bibitem{supercond} 
J. M. Gambetta, J. M. Chow, and M. Steffen, ``Building logical qubits in a superconducting quantum computing system,'' \textit{npj Quantum Inf}, vol. 3, no. 2, 2017. doi: 10.1038/s41534-016-0004-0.

\bibitem{neutral}
L. Henriet, L. Beguin, A. Signoles, T. Lahaye, A. Browaeys, G. O. Reymond, C. Jurczak, ``Quantum computing with neutral atoms,'' \textit{Quantum}, vol. 4, no. 327, 2020. doi: 	10.22331/q-2020-09-21-327.

\bibitem{ion-trap}
S. Weidt, J. Randall, S. C. Webster, K. Lake, A. E. Webb, I. Cohen, T. Navickas, B. Lekitsch, A. Retzker, and W. K. Hensinger, ``Trapped-Ion Quantum Logic with Global Radiation Fields,'' \textit{Phys. Rev. Lett.}, vol. 117, no. 22, pp. 220501, 2016. doi: 10.1103/PhysRevLett.117.220501. 

\bibitem{photonic}
D, Niemietz, P. Farrera, S. Langenfeld, and G. Rempe, ``Nondestructive detection of photonic qubits,'' \textit{Nature}, vol. 591, pp. 570–574, 2021. doi: 10.1038/s41586-021-03290-z.

\bibitem{NV-cite}
F. Jelezko, J. Wrachtrup, ``Single defect centres in diamond: A review,'' \textit{Special Issue: Selected Topics in Physics and Applications of CVD Diamond}, vol. 203, no. 13, pp. 3207-3225, 2006. doi: 10.1002/pssa.200671403.

\bibitem{Dirac} P. A. Dirac, ``The principles of Quantum mechanics,'' \textit{Oxford University Press}, 1982.

\bibitem{introQIC} H. K. Lo, S. Popescu, and T. Spiller, ``Introduction to Quantum Computation and Information,'' \textit{World Scientific}, 1998. doi: https://doi.org/10.1142/3724.

\bibitem{Einstein} M. Born, ``The Born-Einstein letters,'' Walker, 1971.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 79 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{qkd1} R. Bedington, J.M. Arrazola, and A. Ling, ``Progress in satellite quantum key distribution,'' \textit{npj Quantum Inf}, vol. 3, no. 30, 2017. doi:10.1038/s41534-017-0031-5.

\bibitem{qkd2} R. Renner, ``Security of Quantum Key Distribution,'' \textit{PhD dissertation}, Swiss Federal Institute of Tech., Zurich, Switzerland, 2005. arXiv:quant-ph/0512258.

\bibitem{qkd3} A. Cabello, ``Quantum Key Distribution in the Holevo Limit,'' \textit{Phys. Rev. Letters}, vol. 85, no. 26, pp. 5635, 2000. doi: 10.1103/PhysRevLett.85.5635.

\bibitem{telep1} C. H. Bennett, G. Brassard, C. Crépeau, R. Jozsa, A. Peres, and W. K. Wootters, ``Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels,''  \textit{Phys. Rev. Letters}, vol. 70, no. 13, pp. 1895-1899, 1993. doi: 10.1103/PhysRevLett.70.1895.

\bibitem{telep2} D. Bouwmeester, J. W. Pan, K. Mattle, M. Eibl, H. Weinfurter, and A. Zeilinger, ``Experimental quantum teleportation,'' \textit{Nature}, vol. 390, pp. 575–579, 1997. doi:10.1038/37539.

\bibitem{superdense1} C. H. Bennett S. J. Wiesner, ``Communication via one- and two-particle operators on Einstein-Podolsky-Rosen states,''  \textit{Phys. Rev. Letters}, vol. 69, no. 20, pp. 2881-2884, 1993. doi: 10.1103/PhysRevLett.69.2881.

\bibitem{superdense2} J. Barreiro, TC. Wei, and P. Kwiat, ``Beating the channel capacity limit for linear photonic superdense coding,'' \textit{Nature Phys}, vol. 4, pp. 282–286, 2008. doi: 10.1038/nphys919.

\bibitem{josurev} J. Etxezarreta Martinez, P. Fuentes, P. M. Crespo, and J. Garcia-Frias, ``Approximating Decoherence Processes
for the Design and Simulation of
Quantum Error Correction Codes in
Classical Computers,'' \textit{IEEE Access}, vol. 8, pp. 172623-172643, 2020. doi: 10.1109/ACCESS.2020.3025619.

\bibitem{reviewPat}
P. Fuentes, J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Frias, ``Degeneracy and its impact on the decoding of sparse quantum codes,'' \emph{IEEE Access} vol. 9, pp. 89093-89119, 2021. doi: 10.1109/ACCESS.2021.3089829.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 88 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{penrose}
R.Penrose, ``Application of negative dimensional tensors,''  \textit{Combinatorial Mathematics and Its Applications}, Academic Press, pp. 221-224, 1971. online: http://homepages.math.uic.edu/~kauffman/Penrose.pdf.

\bibitem{Knil1}
E. Knill and R. Laflamme, ``A theory of quantum error-correcting codes,'' \textit{Phys. Rev. A}, vol. 55, no. 2, pp. 900-911, 1997. doi: 10.1103/PhysRevA.55.900.

\bibitem{Bennett1}
C. Bennett, D. DiVincenzo, J. Smolin, and W. Wootters, ``Mixed state entanglement and quantum error correction,'' \textit{Phys. Rev. A}, vol. 54, no. 5, pp. 3824-3851, 1996. doi: 10.1103/PhysRevA.54.3824.

\bibitem{scheme-decoherence}
P. W. Shor, ``Scheme for reducing decoherence in quantum computer memory,'' \textit{Phys. Rev. A}, vol. 52, no. 4, pp. R2493-R2496, 1995. doi: 10.1103/PhysRevA.52.R2493.

\bibitem{GotKnill}
D. Gottesman, ``The Heisenberg representation of quantum computers,'' \textit{Proc. Int. Conf. Group Theoretic Methods Phys.}, pp. 1–20, 1998. arXiv:quant-ph/9807006.

\bibitem{Shannon} C. E. Shannon, ``A mathematical theory of communication,'' \textit{Bell System Technical Journal}, vol. 27, pp. 379-423, 1948.

\bibitem{nonbinblock1}
J. Hou, P. H. Siegel, L. B. Milstein and H. D. Pfister, ``Capacity-approaching bandwidth-efficient coded modulation schemes based on low-density parity-check codes,'' \textit{IEEE Transactions on Information Theory}, vol. 49, no. 9, pp. 2141-2155, 2003, doi: 10.1109/TIT.2003.815777.

\bibitem{nonbinblock2}
A. Bennatan and D. Burshtein, ``On the application of LDPC codes to arbitrary discrete-memoryless channels,'' \textit{IEEE Transactions on Information Theory}, vol. 50, no. 3, pp. 417-438, 2004, doi: 10.1109/TIT.2004.824917.

\bibitem{nonbinblock3}
A. Bennatan and D. Burshtein, ``Design and analysis of nonbinary LDPC codes for arbitrary discrete-memoryless channels,'' \textit{IEEE Transactions on Information Theory}, vol. 52, no. 2, pp. 549-583, 2006, doi: 10.1109/TIT.2005.862080.

\bibitem{nonbinblock4}
E. Hof, I. Sason and S. Shamai, ``Performance Bounds for Nonbinary Linear Block Codes Over Memoryless Symmetric Channels,'' \textit{IEEE Transactions on Information Theory}, vol. 55, no. 3, pp. 977-996, 2009, doi: 10.1109/TIT.2008.2011443.


\bibitem{ham14}
R. W. Hamming, ``Error detecting and error correcting Codes,'' \textit{The Bell System technical journal}, vol. 29, no. 2, pp. 147-160, 1950. doi: 10.1002/j.1538-7305.1950.tb00463.x.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 98 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{ldpc1} R. Gallager, ``Low-density parity-check codes,'' in \emph{IRE Transactions on Information Theory}, vol. 8, no. 1, pp. 21-28, January 1962, doi: 10.1109/TIT.1962.1057683.

\bibitem{ldpc2} R. G. Gallager, ``Low-Density Parity-Check Codes,'' \emph{M.I.T Press}, 1963.

\bibitem{ldpc3} D. J. C. MacKay, ``Good error-correcting codes based on very sparse matrices,'' \emph{IEEE Transactions on Information Theory}, vol. 45, no. 2, pp. 399-431, March 1999, doi: 10.1109/18.748992.

\bibitem{ldpc4}
D. J. C. MacKay and R. M. Neal, ``Near Shannon limit performance of low density parity check codes,'' \textit{Electronics Letters }, vol. 33, no. 6, pp. 457 - 458, 1997. online: https://www.semanticscholar.org/paper/Near-Shannon-Limit-Performance-of-Low-DensityParity-CodesDavid-C./27b1996dc57dd04f22a4b3aee4d0364855db4675.

\bibitem{ldpc5}
S. Y. Chung, G. D. Forney, T. J. Richardson and R. Urbanke, ``On the design of low-density parity-check codes within 0.0045 dB of the Shannon limit,'' \textit{IEEE Communications Letters}, vol. 5, no. 2, pp. 58-60, 2001. doi: 10.1109/4234.905935.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 103 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{ldpc6}
L. Chen, J. Xu, I. Djurdjevic, and S. Lin, ``Near-Shannon-limit quasi-cyclic low-density parity-check codes,'' \textit{IEEE Transactions on Communications}, vol. 52, no. 7, pp. 1038 - 1042, 2004. doi: 10.1109/TCOMM.2004.831353.

\bibitem{Tanner1}
R. M. Tanner, ``A recursive approach to low complexity codes,'' \textit{IEEE Transactions on Information Theory}, vol. 27, no.5, pp. 533-547, 1981. doi: 10.1109/TIT.1981.1056404.

\bibitem{Tanner2}
N. Wiberg, H.-A. Loeliger, and R. Kotter, ``Codes and iterative decoding on general graphs,'' \textit{Proceedings of 1995 IEEE International Symposium on Information Theory}, pp. 468, 1995. doi: 10.1109/ISIT.1995.550455.

\bibitem{imagra}
I. Granada, ``Rate compatible joint-source channel coding for poin-to-point and multiple access channels,'' \textit{PhD dissertation}, Tecnun - University of Navarra, San Sebastian, EUS, Spain, 2021. online: https://dadun.unav.edu/handle/10171/61091.

\bibitem{factor-cite1} C. Berrou, A. Glavieux and P. Thitimajshima, ``Near Shannon limit error-correcting coding and decoding: Turbo-codes. 1,'' in \emph{Proceedings of ICC '93 - IEEE International Conference on Communications}, Geneva, Switzerland, 1993, pp. 1064-1070 vol.2, doi: 10.1109/ICC.1993.397441.

\bibitem{factor-cite2} D. J. C. MacKay, ``Good error-correcting codes based on very sparse matrices,'' \textit{IEEE Transactions on Information Theory}, vol. 45, no. 2, pp. 399-431, 1999. doi: 10.1109/18.748992.


\bibitem{cp2_mackay}  D. J. Mackay, ``Information Theory, Inference, and Learning Algorithms,'' \emph{Cambridge University Press}, 2003. USA.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 110 %%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{nonbin1}
D. Declercq and M. Fossorier, ``Decoding Algorithms for Nonbinary LDPC Codes Over GF(q),'' \textit{IEEE Transactions on Communications}, vol. 55, no. 4, pp. 633 - 643, 2007. doi: 10.1109/TCOMM.2007.894088.

\bibitem{nonbin2}
V. S. Ganepola, R. A. Carrasco, I. J. Wassell, and S. Le Goff, ``Performance study of non-binary LDPC Codes over GF(q),'' \textit{6th International Symposium on Communication Systems, Networks and Digital Signal Processing}, pp. 585-589, 2008. doi: 10.1109/CSNDSP.2008.4610743.

\bibitem{LUT1} S. Lin and D. J. Costello, ``Error Control Coding: Fundamentals and Applications,'' \textit{Prentice-Hall}, 2011. 

\bibitem{MLhard}
E. R. Berlekamp, R. J. McEliece, and H. van Tilborg, ``On the inherent intractability of certain coding
problems,'' \emph{IEEE Trans. Info. Theor.}, vol. 24, no. 3, pp. 384 - 386, 1978.

\bibitem{class-IT} T. M. Cover and J. A. Thomas, ``Elements of Information Theory,'' John Wiley Sons, Hoboken, New Jersey, 2006.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 116 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{catalytic}
 T. A. Brun, I. Devetak, and M. Hsieh, ``Catalytic Quantum Error Correction,'' \textit{IEEE Trans. Inf. Theory}, vol. 60, no. 6, pp. 3073-3089, 2014. doi: 10.1109/TIT.2014.2313559
 
 
\bibitem{EAQECC}
T. Brun, I. Devetak, and M. Hsieh, ``Correcting Quantum Errors with Entanglement,'' \textit{Science}, vol. 314, no. 5798, pp. 436-439, 2006. doi: 	10.1126/science.1131563.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 118 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \bibitem{group1} A. R. Calderbank, E. M. Rains, P. M. Shor and N. J. A. Sloane, ``Quantum error correction via codes over GF(4),'' \textit{IEEE Transactions on Information Theory}, vol. 44, no. 4, pp. 1369-1387, 1998. doi: 10.1109/18.681315.

\bibitem{group2} N. Rengaswamy, R. Calderbank, S. Kadhe and H. D. Pfister, ``Logical Clifford Synthesis for Stabilizer Codes,'' \textit{IEEE Transactions on Quantum Engineering}, vol. 1, pp. 1-17, 2020, 2020. doi: 10.1109/TQE.2020.3023419.


\bibitem{QEClidar} D. Lidar, and T. Brun, ``Quantum Error Correction,'' \textit{Cambridge: Cambridge University Press}, 2013. doi: 10.1017/CBO9781139034807.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 121 %%%%%%%%%%%%%%%%%%%%%%

\bibitem{degen-improv1}
C. Crépeau, D. Gottesman, and A. Smith, ``Approximate Quantum Error-Correcting Codes and Secret Sharing Schemes,'' \textit{Advances in Cryptology – EUROCRYPT 2005.} Springer, 2005. doi: 10.1007/11426639\_17.

\bibitem{degen-improv2}
G. Smith and J. A. Smolin, ``Degenerate Quantum Codes for Pauli Channels,'' \textit{Phys. Rev. Lett.}, vol. 98, no.3, pp. 030501, 2007. doi: 10.1103/PhysRevLett.98.030501.

\bibitem{TPS}
 N. Raveendran and B. Vasić, ``Trapping Sets of Quantum LDPC Codes,'' arXiv:2012.15297, 2020
 
 \bibitem{mod-BP} %93
A. Rigby, J. C. Olivier, and P. Jarvis, ``Modified belief propagation decoders for quantum low-density parity-check codes,'' \textit{Physical Review A}, vol. 100, no. 1, pp. 012330, 2019. doi: 	10.1103/PhysRevA.100.012330.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 125 %%%%%%%%%%%%%%%%%%%%%%%%
 
 \bibitem{cycle14}
P. Hu and H. Zhao, ``Improved method for detecting the short cycles of LDPC codes,'' \textit{2010 IEEE International Conference on Information Theory and Information Security}, pp. 841-844, 2010. doi: 10.1109/ICITIS.2010.5689706.

\bibitem{cycle15}
M. Karimi and A. H. Banihashemi, ``Counting Short Cycles of Quasi Cyclic Protograph LDPC Codes,'' \textit{IEEE Communications Letters}, vol. 16, no.3, pp. 400-403, 2012. doi: 10.1109/LCOMM.2012.020212.112311.

\bibitem{cycle16}
M. Karimi and A. H. Banihashemi, ``On the Tanner Graph Cycle Distribution of Random LDPC, Random Protograph-Based LDPC, and Random Quasi-Cyclic LDPC Code Ensembles,'' \textit{ IEEE Trans. on Information Theory}, vol. 64, no.6, pp. 4438-4451, 2018. doi: 10.1109/TIT.2018.2805906.


\bibitem{cycle1}
T. Tian, C. R. Jones, J. D. Villasenor, and  R. D. Wesel, ``Selective avoidance of cycles in irregular LDPC code construction,'' \textit{IEEE Trans. on Communications}, vol. 52, no.8, pp. 1242-1247, 2004. doi: 10.1109/TCOMM.2004.833048.


\bibitem{cycle2}
J. L. Kim, U.N. Peled, I. Perepelitsa, V. Pless, and S. Friedland, ``Explicit construction of families of LDPC codes with no 4-cycles,'' \textit{IEEE Trans. Inform. Theory}, vol. 50, no.10, pp. 2378-2388, 2004.  doi: 10.1109/TIT.2004.834760.

\bibitem{cycle3}
D. V. Nguyen, S. K. Chilappagari, M. W. Marcellin, and B. Vasic, ``On the Construction of Structured LDPC Codes Free of Small Trapping Sets,'' \textit{IEEE Trans. Inform. Theory}, vol. 58, no.4, pp. 2280 - 2302, 2012. doi: 10.1109/TIT.2011.2173733.

\bibitem{cycle4}
G. Lechner, ``The effect of cycles on binary message-passing decoding of LDPC codes,'' \textit{2010 Australian Communications Theory Workshop (AusCTW)}, pp. 43-47, 2010. doi: 10.1109/AUSCTW.2010.5426759.

\bibitem{cycle5}
J. A. McGowan and R. C. Williamson, ``Loop removal from LDPC codes,'' \textit{Proceedings 2003 IEEE Information Theory Workshop}, pp. 230-233, 2003. doi: 10.1109/ITW.2003.1216737.


\bibitem{hag1}
M. Hagiwara and H. Imai, ``Quantum quasi-cyclic LDPC codes,'' \textit{Proc.
IEEE Int. Symp. Inf. Theory}, pp. 806–810, 2007. doi: 10.1109/ISIT.2007.4557323.

\bibitem{hag2}
M. Hagiwara, K. Kasai, H. Imai, and K. Sakaniwa, ``Spatially coupled quasi-cyclic quantum LDPC codes,'' \textit{Proc. IEEE Int. Symp. Inf. Theory}, pp. pp. 638–642, 2011. doi: 10.1109/ISIT.2011.6034208.

\bibitem{hag3}
K. Kasai, M. Hagiwara, H. Imai, and K. Sakaniwa, ``Non-binary quasi-cyclic quantum LDPC codes,'' \textit{IEEE Int. Symp. Inf. Theory Proceedings}, 637-657, 2011. doi: 10.1109/ISIT.2011.6034212.

\bibitem{hag4}
K. Kasai, M. Hagiwara, H. Imai and K. Sakaniwa, ``Quantum Error Correction Beyond the Bounded Distance Decoding Limit,'' \textit{IEEE Transactions on Information Theory}, vol. 58, no. 2, pp. 1223-1230, 2012. doi: 10.1109/TIT.2011.2167593.

\bibitem{short-cycle-improv}
K. Chung and J. Heo, ``Improved Belief Propagation (BP) Decoding for LDPC Codes with a large number of short cycles,'' \textit{2006 IEEE 63rd Vehicular Technology Conference}, pp. 1464-1466, 2006. doi: 10.1109/VETECS.2006.1683078.

\bibitem{efb}
Y. Wang, B. C. Sanders, B. Bai and X. Wang, ``Enhanced Feedback Iterative Decoding of Sparse Quantum Codes,'' \textit{IEEE Trans. Inform. Theory}, vol. 58, no. 2, pp. 1231-1241, 2012. doi: 10.1109/TIT.2011.2169534.

\bibitem{TPS-thes}
N. Raveendran, ``Trapping Sets of Iterative Decoders for Quantum and Classical Low-Density Parity-Check Codes,''\textit{PhD Dissertation}, The University of Arizona, 2021. online: https://www.proquest.com/docview/2598659782?pq-origsite=gscholar\&fromopenview=true.

\bibitem{osd1}  P. Panteleev and G. Kalachev, ``Degenerate quantum LDPC codes with good ﬁnite length performance,'' arXiv:1904.02703, 2019. 

\bibitem{osd2}  J. Roffe, D. R. White, S. Burton, and E. T. Campbell, ``Decoding Across the Quantum LDPC Code Landscape,'' \textit{Phys. Rev. Research}, vol. 2, no. 4, pp. 043423, 2020. doi: 10.1103/PhysRevResearch.2.043423.

\bibitem{refined}  Kao-Yueh Kuo and Ching-Yi Lai, ``Refined Belief Propagation Decoding of Sparse-Graph Quantum Codes,'' \textit{IEEE Journal on Selected Areas in Information Theory}, vol. 1, no. 2, pp. 487-498, 2020. doi: 10.1109/JSAIT.2020.3011758.	

\bibitem{exploiting} K.-Y. Kuo and C.-Y. Lai, ``Exploiting degeneracy in belief propagation
decoding of quantum codes,'' 2021. arXiv:2104.13659.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 141 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibitem{jgf3} J. Garcia-Frias and K. Liu, ``Design of near-optimum quantum error-correcting codes based on generator and parity-check matrices of LDGM codes,'' \textit{42nd. Annual Conference on Information Sciences and Systems}, pp. 562-567, 2008. doi: 10.1109/CISS.2008.4558588.


\bibitem{Til} T. Camara, H. Ollivier and J. Tillich, ``A class of quantum LDPC codes: construction and performances under iterative decoding,'' \textit{2007 IEEE International Symposium on Information Theory}, 2007, pp. 811-815, doi: 10.1109/ISIT.2007.4557324.

\bibitem{bab11} Z. Babar, P. Botsinis, D. Alanis, S. Xin Ng and L. Hanzo, ``Construction of Quantum LDPC Codes From Classical Row-Circulant QC-LDPCs,'' \textit{IEEE Communications Letters}, vol. 20, no. 1, pp. 9-12, 2016, doi: 10.1109/LCOMM.2015.2494020.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 145 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Benny} K. Kuo and C. Lu, ``A further study on the encoding complexity of quantum stabilizer codes,'' \textit{2010 International Symposium On Information Theory \& Its Applications}, 2010, pp. 1041-1044, doi: 10.1109/ISITA.2010.5649496.

\bibitem{Wilde} M. Wilde, ``Logical operators of quantum codes,'' \textit{Phys. Rev. A}, vol. 79, pp. 062322, 2009. doi: 10.1103/PhysRevA.79.062322.

\bibitem{patrick2} P. Fuentes, J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Frias, ``Design of LDGM-based quantum codes for asymmetric quantum channels,'' \textit{Phys. Rev. A}, vol. 103, pp. 022617, 2021. doi: 10.1103/PhysRevA.103.022617.

\bibitem{patrick3}
P. Fuentes, J. Etxezarreta Martinez, P. M. Crespo, and J. Garcia-Fr\'ias, ``Performance of non-CSS LDGM-based quantum codes over the Misidentified Depolarizing Channel,'' \textit{IEEE International Conference on Quantum Computing and Engineering (QCE20)}, 2020. doi:10.1109/QCE49297.2020.00022.

\bibitem{MonteCarlo} M. Jeruchim, ``Techniques for Estimating the Bit Error Rate in the Simulation of Digital Communication Systems,'' \emph{IEEE J. Selected Areas Commun,} {\bf 1984}, {\em 2},~153--170. doi: 10.1109/JSAC.1984.1146031.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 150 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{rewiring}
 K. R. Colladay and E. J. Mueller, ``Rewiring stabilizer codes,'' \textit{New J. Phys.}, vol. 20, pp. 083030, 2018. doi: 10.1088/1367-2630/aad8dd.
 
\bibitem{classicaltoquantum} Z. Babar, D. Chandra, H. V. Nguyen, P. Botsinis, D. Alanis, S. X. Ng, and L. Hanzo, ``Duality of Quantum and Classical Error Correction Codes: Design Principles and Examples,'' \textit{IEEE Communications Surveys Tutorials}, vol. 29, no. 1, pp. 970-1010, 2019. doi: 10.1109/COMST.2018.2861361.
 
\bibitem{newcite} Z. Babar, P. Botsinis, D. Alanis, S. X. Ng and L. Hanzo, ``The Road From Classical to Quantum Codes: A Hashing Bound Approaching Design Procedure,'' \textit{IEEE Access}, vol. 3, pp. 146-176, 2015. doi: 10.1109/ACCESS.2015.2405533.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QLDPC - 153

\bibitem{turbo2} C. Berrou, R. Pyndiah, P. Adde, C. Douillard and R. Le Bidan, ``An overview of turbo codes and their applications,'' \textit{The European Conference on Wireless Technology}, pp. 1-9, 2005. doi: 10.1109/ECWT.2005.1617639.

\bibitem{LDPCshan1}
D. J. C. MacKay and R. M. Neal, ``Near Shannon limit performance of low density parity check codes,'' \textit{Electronics Letters }, vol. 33, no. 6, pp. 457 - 458, 1997. online: https://www.semanticscholar.org/paper/Near-Shannon-Limit-Performance-of-Low-DensityParity-CodesDavid-C./27b1996dc57dd04f22a4b3aee4d0364855db4675.

\bibitem{LDPCshan2}
S. Y. Chung, G. D. Forney, T. J. Richardson and R. Urbanke, ``On the design of low-density parity-check codes within 0.0045 dB of the Shannon limit,'' \textit{IEEE Communications Letters}, vol. 5, no. 2, pp. 58-60, 2001. doi: 10.1109/4234.905935.

\bibitem{LDPCshan3}
L. Chen, J. Xu, I. Djurdjevic, and S. Lin, ``Near-Shannon-limit quasi-cyclic low-density parity-check codes,'' \textit{IEEE Transactions on Communications}, vol. 52, no. 7, pp. 1038 - 1042, 2004. doi: 10.1109/TCOMM.2004.831353.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 157

\bibitem{EXITQTC} 
Z. Babar, S. X. Ng, and L. Hanzo, ``EXIT-Chart-Aided Near-Capacity Quantum Turbo Code Design,'' \textit{IEEE Transactions on Vehicular Technology}, vol. 64, pp. 866-875, 2015. doi: 10.1109/TVT.2014.2328638.

\bibitem{EAQIRCC} 
H. V. Nguyen, Z. Babar, D. Alanis, P. Botsinis, D. Chandra, S. X. Ng, and L. Hanzo, ``EXIT-Chart Aided Quantum Code Design Improves the Normalised Throughput of Realistic Quantum Devices,'' \textit{IEEE Access}, vol. 4, pp. 10194-10209, 2016. doi: 10.1109/ACCESS.2016.2591910.

\bibitem{QSBC} 
D. Chandra, Z. Babar, S. X. Ng, and L. Hanzo, ``Near-Hashing-Bound Multiple-Rate Quantum Turbo Short-Block Codes,'' \textit{IEEE Access}, vol. 7, pp. 52712-52730, 2019. doi: 10.1109/ACCESS.2019.2911515.

\bibitem{fault11}
J. Preskill, ``Fault-tolerant quantum computation,'' 1997. arXiv:quant-ph/9712048

\bibitem{fault22} R. Chao abd B.W. Reichardt, ``Fault-tolerant quantum computation with few qubits,'' \textit{npj Quantum Information}, vol. 4, no. 42, 2018. doi: 10.1038/s41534-018-0085-z.

\bibitem{classicalLDGM}
T. R. Oenning and J. Moon, ``A low-density generator matrix interpretation of parallel concatenated single bit parity codes,'' \textit{IEEE Transactions on Magnetics}, vol. 37, pp. 737-741, 2001. doi: 10.1109/20.917609.


\bibitem{jgf4} K. Liu and J. Garcia-Frias, ``Optimization of LDGM-based quantum codes using Density Evolution,'' \textit{48th Annual Allerton Conference on Communication, Control, and Computing}, 2010. doi: 10.1109/ALLERTON.2010.5707001.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 164 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{EXITRCMLDGM} 
I. Granada, P. M. Crespo, and J. Garcia-Frías, ``Asymptotic BER EXIT chart analysis for high rate codes based on the parallel concatenation of analog RCM and digital LDGM codes,'' EURASIP J Wireless Com Network, vol. 11, 2019. doi: 10.1186/s13638-018-1330-z.

\bibitem{BWTRCMLDGM} 
I. Granada, P. M. Crespo, and J. Garcia-Frías, ``Combining the Burrows-Wheeler Transform and RCM-LDGM Codes for the Transmission of Sources with Memory at High Spectral Efficiencies,'' Entropy, vol. 21, pp. 378, April 2019. doi: 10.3390/e21040378.

\bibitem{Wilde1}
M. M. Wilde, ``Quantum Information Theory,'' \textit{Cambridge Univ. Press}, Cambridge, 2013. doi: https://doi.org/10.1017/CBO9781139525343.

\bibitem{josuarxiv}
J. Etxezarreta Martinez, P. Fuentes, P. M. Crespo, and J. Garcia-Frias, ``Quantum outage probability for time-varying quantum channels,'' \textit{Physical Review A}, vol. 105, pp. 012432, 2022. doi: 	10.1103/PhysRevA.105.012432.

\bibitem{parallelshannon} W. Zhong, H. Chai and J. Garcia-Frias, ``Approaching the shannon limit through parallel concatenation of regular LDGM codes,'' in \emph{Proceedings. International Symposium on Information Theory}, 2005. ISIT 2005., Adelaide, SA, Australia, 2005, pp. 1753-1757, doi: 10.1109/ISIT.2005.1523646.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 182 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{doping} 
S. ten Brink, ``Code doping for triggering iterative decoding convergence,'' \emph{Proceedings. 2001 IEEE International Symposium on Information Theory,} Washington, DC, USA, 2001. doi: 10.1109/ISIT.2001.936098.

\bibitem{jgf5}
Kejing Liu and J. Garcia-Frias, ``Asymptotic analysis of LDGM-based quantum codes,'' \textit{43rd Annual Conference on Information Sciences and Systems}, pp. 87-92, 2009. doi: 10.1109/CISS.2009.5054696.

\bibitem{serialLDGM}
W. Zhong and J. Garcia-Frias, ``LDGM Codes for Channel Coding and
Joint Source-Channel Coding of Correlated Sources,'' \textit{EURASIP Journal on Applied Signal Processing}, vol. 2005, no. 6, pp. 942-953, May 2005. doi: 10.1109/ICIP.2003.1247031.

\bibitem{first-impact}
Y. Xie, J. Li, R. Malaney, and J. Yuan, ``Channel identification and its impact on quantum LDPC code performance,'' \textit{Australian Communications Theory Workshop (AusCTW)}, pp. 140-144, 2012. doi: 10.1109/AusCTW.2012.6164921.

\bibitem{current}
Y. Xie, J. Li, R. Malaney, and J. Yuan, ``Improved quantum LDPC decoding strategies for the misidentified quantum depolarization channel,'' \textit{24th European Signal Processing Conference (EUSIPCO)}, pp. 493-497, 2016. doi: 10.1109/EUSIPCO.2016.7760297.

\bibitem{fissh1}
J. Li, H. Liu, Z. Wang, and Xuexi Yi, ``Cramér-Rao bound and quantum parameter estimation with non-Hermitian systems,'' 2021. arXiv:2103.07099.

\bibitem{cram1}
S. L. Braunstein and C. M. Caves, ``Statistical distance and the geometry of quantum states,'' \textit{Phys. Rev. Lett.}, vol. 72, no. 22, pp. 3439-3443, 1994. doi: 10.1103/PhysRevLett.72.3439.

\bibitem{lastcite}
D. Collins and J. Stephens, ``Depolarizing-channel parameter estimation using noisy initial states,'' \textit{Physical Review A}, vol. 92, pp. 032324, 2015. doi: 10.1103/PhysRevA.92.032324.

\bibitem{probes} 
A. Fujiwara, ``A Quantum channel identification problem,'' Physical Review A, vol. 63, pp. 042304, 2001. doi: 10.1103/PhysRevA.63.042304. 

\bibitem{superconducting-josu}
J. Etxezarreta Martinez, P. Fuentes, P. M. Crespo, and J. Garcia-Frias, ``Time-varying quantum channel models for superconducting qubits,'' \textit{npj Quantum Inf}, vol. 7, no. 115, 2021. doi: 10.1038/s41534-021-00448-5.

\bibitem{josuconf}
J. Etxezarreta Martinez, P. Fuentes, P. M. Crespo, and J. Garcia-Fr\'ias, ``Pauli channel online estimation protocol for quantum turbo codes,'' \textit{IEEE International Conference on Quantum Computing and Engineering (QCE20)}, pp. 102-108, 2020. doi: 10.1109/QCE49297.2020.00023.

\bibitem{asymmetry-1} 
L. Ioffe and M. Mézard, ``Asymmetric quantum error-correcting codes,'' \textit{Physical Review A}, vol. 75, no. 3, pp. 032345, 2007. doi: 10.1103/PhysRevA.75.032345.


\bibitem{model-asymmetry-1} 
F Schmidt-Kaler, S Gulde, M Riebe1, T Deuschle, A Kreuter, G Lancaster, C Becher, J Eschner, H Häffner and R Blatt, ``The coherence of qubits based on single Ca+ ions,'' \textit{Journal of Physics B: Atomic, Molecular Opt. Phys.}, vol. 36, no. 623, 2013. doi: 10.1088/0953-4075/36/3/319.

\bibitem{model-asymmetry-2} 
 L. M. K. Vandersypen, M. Steffen, G. Breyta, C. S. Yannoni, M. H. Sherwood, and I. L. Chuang, ``Experimental realization of Shor's quantum factoring algorithm using nuclear magnetic resonance,'' \textit{Nature}, vol. 414, pp. 883–887, 2001. doi: 10.1038/414883a.

\bibitem{model-asymmetry-3} 
A. M. Tyryshkin, J. J. L. Morton, S. C. Benjamin2, A. Ardavan, G. A. D. Briggs, J. W. Ager and S. A. Lyon, ``Coherence of spin qubits in silicon,'' \textit{Journal of Physics: Condensed Matter}, vol. 18, no. 21, pp. 783-794, 2006. doi: 10.1088/0953-8984/18/21/s06.

 \bibitem{model-asymmetry-4} 
 J. R. Petta, A. C. Johnson, J. M. Taylor, E. A. Laird, A. Yacobym, D. Lukinc, M. Marcus, P. Hanson and A. C. Gossard, ``Coherent Manipulation of Coupled Electron Spins in Semiconductor Quantum Dots,'' \textit{Science}, vol. 309, no. 5744, pp. 2180-2184, 2005. doi: 10.1126/science.1116955.

 
 \bibitem{model-asymmetry-5} 
 P. Bertet, I. Chiorescu, G. Burkard, K. Semba, C. Harmans, D. P. DiVincenzo, and J. Mooij, ``Dephasing of a superconducting qubit induced by photon noise,'' \textit{Physical Review Letter}, vol. 95, no. 25, pp. 257002, 2005. doi: 10.1103/PhysRevLett.95.257002.
 
  \bibitem{asymmetry-2}
 H. V. Nguyen, Z. Babar, D. Alanis, P. Botsinis, D. Chandra, S. X. Ng, and L. Hanzo, ``EXIT-Chart Aided Quantum Code Design Improves the Normalised Throughput of Realistic Quantum Devices,'' \textit{IEEE Access}, vol. 4, pp. 10194-10209, 2016. doi: 10.1109/ACCESS.2016.2591910.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 183 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{short-asym} 
M. Chiani and L. Valentini, ``Short Codes for Quantum Channels With One Prevalent Pauli Error Type,'' \textit{IEEE Journal on Selected Areas in Information Theory}, vol. 1, no. 2, pp. 480-486, 2020. doi: 10.1109/JSAIT.2020.3012827.

\bibitem{alpha1} 
P. K. Sarvepalli, A. Klappenecker, and M. Rötteler, ``Asymmetric quantum codes: constructions, bounds and performance,'' \textit{Proceedings of the Royal Society London A}, vol. 465, no. 2105, pp. 1645-1672, 2009. doi: 10.1098/rspa.2008.0439.

\bibitem{alpha2} 
Z. W. E. Evans, A. M. Stephens, J. H. Cole, and L. C. L. Hollenberg, ``Error correction optimisation in the presence of X/Z asymmetry,'' 2007. arXiv:0709.3875.

\bibitem{alpha3} 
 A. M. Stephens, Z. W. E. Evans, S. J. Devitt, and L. C. L. Hollenberg, ``Asymmetric quantum error correction via code conversion,'' \textit{Physical Review A}, vol. 77, no.6, pp. 062335, 2008. doi: 10.1103/PhysRevA.77.062335.

 
\bibitem{time} 
 C. P. Williams and S. H. Clearwater, ``Explorations in Quantum Computing,'' \textit{Springer}, London, 2011. online: 10.1007/978-1-84628-887-6.
 
\bibitem{eurasip}
F. J. Vazquez-Araujo, M. Gonzalez-Lopez, L. Castedo, and J. Garcia-Frias, ``Serially-Concatenated LDGM Codes for MIMO Channels,'' \textit{IEEE Transactions on Wireless Communications}, vol. 6, no. 8, pp. 2860-2871, 2007. doi: 10.1109/TWC.2007.05651.

\bibitem{klap} P. K. Sarvepalli, A. Klappenecker, and M. Rotteler, ``Asymmetric quantum LDPC codes,'' \textit{IEEE International Symposium on Information Theory}, pp. 305-309, 2008. doi: 10.1109/ISIT.2008.4594997.

\bibitem{34-preskill}
J. Preskill, ``Quantum Computing in the NISQ era and beyond,'' \textit{Quantum}, vol. 2, pp. 1–79, 2018. doi: 10.22331/q-2018-08-06-79.

\bibitem{twirl1}
J. Ghosh, A. G. Fowler, and M. R. Geller, ``Surface code with decoherence: An analysis of three superconducting architectures,'' \textit{Phys. Rev. A}, vol. 86, no. 6, pp. 062318, 2012. doi: 10.1103/PhysRevA.86.062318.

\bibitem{twirl2}
M. Silva, E. Magesan, D. W. Kribs, and J. Emerson, ``Experimentally scalable protocol for identification of correctable codes,'' \textit{Phys. Rev. A}, vol. 78,
no. 1, pp. 012347, 2008. doi: 10.1103/PhysRevA.78.012347.

\bibitem{twirl3}
J. Emerson, M. Silva, O. Moussa, C. Ryan, M. Laforest, J. Baugh,
D. G. Cory, and R. Laflamme, ``Symmetrized characterization of noisy quantum processes,'' \textit{Science}, vol. 317, no. 5846, pp. 1893–1896, 2007. doi: 10.1126/science.1145699.

\bibitem{mem1}
D. Kretschmann and R. F. Werner, ``Quantum channels with memory,''
\textit{Phys. Rev. A}, vol. 72, no. 6, pp. 062323, 2005. doi: 10.1103/PhysRevA.72.062323.

\bibitem{mem2} 
F. Caruso, V. Giovannetti, C. Lupo, and S. Mancini, ``Quantum channels and memory effects,'' \textit{Rev. Mod. Phys.}, vol. 86, no. 4, pp. 1203–1259, 2014. doi: 10.1103/RevModPhys.86.1203.

\bibitem{decoherenceBenchmarking} J. J. Burnett, A. Bengtsson, M. Scigliuzzo, D. Niepce, M. Kudra, P. Delsing, and J. Bylander, ``Decoherence benchmarking of superconducting qubits,'' \emph{npj Quantum Inf.}, vol. 5, no. 54, pp. 1-8, 2019. doi: 10.1038/s41534-019-0168-5.

\bibitem{fluctAPS} S. Schl\"or, J. Lisenfeld, C. M\"uller, A. Bilmes,  A. Schneider, D. Pappas, A. V. Ustinov, and M. Weides, ``Correlating Decoherence in Transmon Qubits: Low Frequency Noise by Single Fluctuators,'' \emph{Phys. Rev. Lett.}, vol. 123, no. 19, pp. 190502, 2019. doi: 10.1103/PhysRevLett.123.190502.

\bibitem{fluctApp} A. Stehli, J. D. Brehm, T. Wolz, P. Baity, S. Danilin, V. Seferai, H. Rotzinger, A. V. Ustinov,  and M. Weides, ``Coherent superconducting qubits from a subtractive junction fabrication process,'' \emph{Applied Physics Letters}, vol. 117, no. 12, pp. 124005, 2020. doi: 10.1063/5.0023533.

\bibitem{temperature}
Z. Wang, S. Shankar, Z. K. Minev, P. Campagne-Ibarcq, A. Narla, and M.H. Devoret, ``Cavity Attenuators for Superconducting Qubits,'' \emph{Phys. Rev. Applied}, vol. 11, no. 1, pp. 014031, 2019. doi: 10.1103/PhysRevApplied.11.014031.

\bibitem{diamondNat}
S. Pirandola, R. Laurenza, C. Lupo et al., ``Fundamental limits to quantum channel discrimination,'' \emph{npj Quantum Inf.}, vol. 5, pp. 50, 2019. doi: 10.1038/s41534-019-0162-y.

\bibitem{FanoDiamond}
G. Benenti and G. Strini, ``Computing the distance between quantum channels: Usefulness of the Fano representation,'' \emph{J. Phys. B: At. Mol. Opt. Phys.}, vol. 43, pp. 215508, 2010. doi: 	10.1088/0953-4075/43/21/215508.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX


\bibitem{URW1} H. Wymeersch, F. Penna, and V. Savic, ``Uniformly reweighted belief propagation: A factor graph approach,'' \emph{Proc. IEEE Int. Symp. Inf. Theory (ISIT)}, pp. 2000–2004, 2012. doi: 10.1109/ISIT.2011.6033905.

\bibitem{URW2} H. Yuan and P. Kam, ``The LLR Metric for q-ary LDPC Codes with MPSK Modulation over Rayleigh Channels with Imperfect CSI,'' \emph{IEEE Transactions on Communications}, vol. 60, no. 7, pp. 1793-1799, 2012. doi: 10.1109/TCOMM.2012.050812.110129.

\bibitem{imagra-nonbin} I. Granada, P. M. Crespo, M. E. Burich and J. Garcia-Frías, ``Rate Compatible Modulation for Correlated Information Sources,'' in IEEE Access, vol. 9, pp. 65449-65465, 2021, doi: 10.1109/ACCESS.2021.3073972.

\bibitem{adj-surf} N. Delfosse and J.-P. Tillich, ``A decoding algorithm for CSS codes using the X/Z correlations,'' \emph{IEEE International Symposium on Information Theory}, pp. 1071–1075, 2014. doi: 10.1109/ISIT.2014.6874997.

\bibitem{class-mismatch1}
N. Merhav, G. Kaplan, A. Lapidoth, and S. Shamai, ``On information rates for mismatched decoders,'' \textit{IEEE Trans. Inform. Theory}, vol. 40, no. 6, pp. 1953–1967, 1994. doi: 10.1109/18.340469.

\bibitem{class-mismatch2}
A. Lapidoth and P. Narayan, ``Reliable communication under channel
uncertainty,'' \textit{IEEE Trans. Inform. Theory}, vol. 44, no. 6, pp. 2148-2177, 1998. doi: 10.1109/18.720535.

\bibitem{class-mismatch3}
A. Ganti, A. Lapidoth, and Ë™I. Emre Telatar, ``Mismatched Decoding Revisited: General Alphabets, Channels with Memory, and the Wide-Band Limit,'' \textit{IEEE Trans. Inform. Theory}, vol. 46, no. 7, pp 2315 - 2328, 2000. doi: 10.1109/18.887846.


\bibitem{tanh}
J. Hagenauer, E. Offer and L. Papke, ``Iterative decoding of binary block and convolutional codes,'' \textit{IEEE Trans. Inform. Theory}, vol. 42, no.2, pp. 429-445, 1996. doi: 10.1109/18.485714.


\bibitem{approx-BP}
T. Richardson and R. Urbanke, ``Modern coding theory,'' \textit{Cambridge University Press}, 2008. doi: 10.1017/CBO9780511791338.

\bibitem{class-aug} A. Rigby, J. Olivier, H. C. Myburgh, C. Xiao, and B. P. Salmon, ``Augmented decoders for LDPC codes,'' \emph{EURASIP Journal on Wireless Communications and Networking 2018}, no. 189, 2018. doi: 10.1186/s13638-018-1203-5. 

\bibitem{class-osd1} M. P. C. Fossorier and S. Lin, ``Soft-Decision Decoding of Linear Block Codes Based on Ordered Statistics,'' \emph{IEEE Transactions on Information Theory}, vol. 41, no. 5, pp. 1379-1396, 1995. doi: 10.1109/18.412683.

\bibitem{serialBP1} J. Zhang and M. P. C. Fossorier, ``Shuffled iterative decoding,'' \emph{IEEE Transactions on Communications}, vol. 53, pp. 209–213, 2005. doi: 10.1109/TCOMM.2004.841982.

\bibitem{serialBP2}  E. Sharon, S. Litsyn, and J. Goldberger, ``Efficient serial message-passing schedules for LDPC decoding,'' \emph{IEEE Trans. Inf. Theory}, vol. 53, pp. 4076–4091, 2007. doi: 10.1109/TIT.2007.907507.

\bibitem{norm1} J. Chen and M. P. C. Fossorier, ``Near optimum universal belief propagation based decoding of low-density parity check codes,'' \emph{IEEE Transactions on Communications}, vol. 50, pp. 406–414, 2002. doi: 10.1109/26.990903. doi: 10.1109/26.990903.

\bibitem{norm2}  J. Chen, A. Dholakia, E. Eleftheriou, M. P. C. Fossorier, and X.-Y. Hu, ``Reduced-complexity decoding of LDPC codes,'' \emph{IEEE Transactions on Communications}, vol. 53, pp. 1288–1299, 2005. doi: 10.1109/TCOMM.2005.852852.

\bibitem{norm3}  M. R. Yazdani, S. Hemati, and A. H. Banihashemi, ``Improving belief
propagation on graphs with cycles,'' \emph{IEEE Communications Letters}, vol. 8, pp.
57–59, 2004. doi: 10.1109/LCOMM.2003.822499.













% 66
















\end{thebibliography}


==> Texs/COVER/abstract.tex <==



% Any communication system is benefited of compressing the information produced by the data sources to its most elementary representation before being transmitted. From an information theoretical perspective this problem is usually separated into two independent subproblems. First, the actual amount of information $H$, called entropy, that the binary source generates is characterized in bits per source symbol. Using an ideally perfect lossless data compression algorithm, exploiting the statistical redundancy of the source symbols the same information can be represented in fewer bits, and the exact amount of bits is given by the entropy of the source. Second, the maximum number of bits per channel symbol that any transmitter can accept if these information bits are to be recovered at the receiver side with low probability of error is characterized by the capacity, $C$, of the channel, given by the maximum of the mutual information between the input and output of the channel, where the maximization is with respect to the input distribution. The algorithms to achieve near the capacity transmission rates are called channel codes. As the Separation Theorem states, reliable communication of the information generated by a source is possible if and only if $H<C$ and it is optimal to solve each of the subproblems individually. However, when considering practical issues like complexity and delay, algorithms that treat the source compression and channel coding in a joint fashion tend to perform better and therefore, are becoming more and more popular. This family of algorithms are called Joint Source-Channel Codes (JSCC). Moreover, the separation problem does not in general hold in multi-user communications.

In this Thesis we consider high-throughput rate compatible Joint Source-Channel Coding (JSCC) schemes based on Rate Compatible Modulation (RCM) codes. These codes achieve JSCC capabilities by embedding source compression into modulation through the generation of multi-level symbols from weighted linear combinations of the input bits. The smooth rate adaptation is achieved seamlessly by varying the number of generated symbols. These two properties makes them advantageous over conventional Adaptive Coded Modulation (ACM) techniques, which usually rely on unrealistic instant and accurate channel estimations, and a limited set of coding and modulation combinations. 

Unfortunately, RCM codes experience performance degradation due to the presence of error floors at high Signal-to-Noise Ratios (SNRs). These error floors can be substantially improved by introducing Low Density Generator Matrix (LDGM) codes in parallel. The main idea is to substitute a few RCM symbols by LDGM coded bits, forming an hybrid coding scheme composed by the parallel concatenation of an analog RCM and a digital LDGM code. The goal of the LDGM symbols is to correct residual errors produced by the RCM. If properly designed, the resulting RCM-LDGM coding scheme achieves good performances while preserving the JSCC and rate adaptation capabilities of RCM codes.


This work investigates insights and new application techniques of these family of codes for point-to-point and multi-user communications. To that end, this thesis is divided in two different parts:

\begin{itemize}
	
	\item The first part of the dissertation considers the point-to-point transmission of a single source. 
	
	We begin by proposing an EXIT chart analysis and a Bit Error Rate (BER) prediction procedure suitable for implementing RCM-LDGM codes. The decoder of these codes is based on the iterative Sum-Product algorithm which exchange information between variable nodes (VN) and the corresponding two types of check nodes: RCM-CN and LDGM-CN. To obtain good codes that achieve near Shannon limit performance one is required to obtain BER versus SNR behaviors for different families of possible code design parameters. For large input block lengths, this could take large amount of simulation time, which is sped up with the designed EXIT procedure.
	
	Then, we consider the problem of implementing high-throughput JSCC schemes for the transmission of binary sources with memory over AWGN channels. Concretely, we propose a coding scheme based on the Burrows-Wheeler Transform (BWT) and RCM-LDGM codes. The proposed scheme utilizes the BWT to convert the original source with memory into a set of independent non-uniform Discrete Memoryless (DMS) binary sources, which are then separately encoded, with optimal rates, using RCM-LDGM codes. The proposed BWT technique outperforms the scheme obtained by attaching the statistical structure of the source to the decoding process in the receiver.
	
	Finally, we consider the transmission of high data rates over additive impulsive noise channels, for which we propose the use of RCM-LDGM codes with an adapted decoder when the channel state information is available at the receiver.
	
	
	\item The second part of the Thesis pays attention to the transmission of multiple information sources over non-orthogonal Multiple Access Channels (MACs). 
	
	We begin by considering that the information sources are uncorrelated and propose a new coding scheme based on the use of an irregular RCM encoder for each user. By properly designing the encoders and taking advantage of the additive nature of the MAC, the joint decoder from the inputs of all the users can be represented by a bipartite graph corresponding to a standard point-to-point RCM structure with certain constraints. Decoding is performed over this bipartite graph utilizing the sum-product algorithm. The proposed scheme allows the simultaneous transmission of a large number of uncorrelated users at high rates, while the decoding complexity is the same as that of standard point-to-point RCM schemes. 
	
	Secondly, we consider that the transmitted information sources are spatially correlated. In this case, it is well known that the system performance is optimized if the codewords are designed to take advantage of the correlation among sources in the MAC. Following this criteria, we propose a novel coding system that makes use of a set of RCM codes that share the same random structure but with each code having its own weight values that are jointly designed to preserve the source correlation in the codewords. At the receiver, non-binary decoding is applied to avoid cycles that arise in the factor graph, which is obtained by jointly considering the source correlation and the RCM codes. We also propose the use of a LDGM codes in parallel with the proposed RCM structures in the MAC aiming to reduce the error floor.
	
	

\end{itemize}

%All in all, this Thesis aims to propose novel high rate communication schemes that achieve rateless joint source-channel coding in a varied number of situations.


